Permutation invariance, partition algebras and large $N$ matrix models

In this thesis we will study matrix models with discrete gauge group $S_N$. We will put these matrix models into a generalized Schur-Weyl duality framework where dual algebras, known as partition algebras, emerge. These form generalizations of the symmetric group algebras -- they are semi-simple finite-dimensional associative algebras with a basis labelled by diagrams. We review the structure and representation theory of partition algebras. These algebras are then used to compute expectation values of $S_N$ invariant observables. This is a step towards studying the emergence of new geometric structures in their Feynman diagram expansion. Matrix models also appear in the form of quantum mechanical models of matrix oscillators. We explore the implications of the Schur-Weyl duality framework to matrix quantum mechanics with permutation symmetry.

==> Chapters/ApxCode.tex <==


    % Prevent overflowing lines due to hard-to-break entities
    \sloppy 
    % Setup hyperref package
%    \hypersetup{
%      breaklinks=true,  % so long urls are correctly broken across lines
%      colorlinks=true,
%      urlcolor=urlcolor,
%      linkcolor=linkcolor,
%      citecolor=citecolor,
%      }
%    % Slightly bigger margins than the latex defaults
%    
%    \geometry{verbose,tmargin=1in,bmargin=1in,lmargin=1in,rmargin=1in}
%    
%    

%    \maketitle
    
    

    % Add a bibliography block to the postdoc
    
    
    

